Graph-Guided Selective Unlearning for Language Models: Controlling Support Routes Beyond Forget Seeds

Enterprises fine-tune language models on proprietary data that may later require removal due to privacy, contractual, or compliance obligations. Selective unlearning removes requested knowledge while preserving model utility, offering a practical alternative to full retraining, but existing methods treat the explicitly identified forget examples as the complete deletion scope. This is insufficient when target knowledge remains recoverable through paraphrases, aliases, or neighboring training examples. We propose GRAPHSU, a graph-guided controller that expands the deletion scope beyond forget seeds by constructing a weighted support-route graph, propagating deletion pressure through it, and applying graded forgetting strengths to high-risk neighbors. On the Task of Fictitious Unlearning (TOFU), a synthetic author-profile question-answering benchmark, and PISTOL, a structural-unlearning benchmark built around interconnected factual samples, with GPT-2 Medium and Llama-3.2-3B-Instruct, GRAPHSU achieves the lowest utility-feasible soft leakage across all deletion settings, reducing leakage by up to 49.5 percentage points over a matched seed-only baseline, demonstrating that effective enterprise unlearning requires controlling support routes, not just forget seeds.

==> appendices/operational_details.tex <==
% Operational appendix for inclusion from main.tex.
% Required in the main preamble:
%   \newcolumntype{L}{>{\raggedright\arraybackslash}X}
% This file assumes that \method, tab:settings, and the appendix mode
% are already defined in main.tex. It intentionally contains no
% \documentclass, package imports, \appendix, \section, or \end{document}.

\subsection{Measurement methodology and operational phases}

We distinguish three phases. \emph{(i) Offline, corpus-level, reusable:} fact extraction,
support-graph construction, and optional GradAlign preprocessing, computed once per corpus and
cached. \emph{(ii) Per deletion request:} request grounding, one- and two-hop support-closure
retrieval, support scoring, actionability/retain-safety filtering, and the model update.
\emph{(iii) Offline validation:} lightweight checkpoint evaluation (development-time) and the full
adversarial route audit. ``Cost'' is wall-clock time unless noted. Only fact extraction issues
external GPT-4.1 calls; all other generations are local. All timings use GPT-2-medium on TOFU on a
single NVIDIA RTX 3090 at seed~42, so the results characterise one consistent, controlled
configuration.

\subsection{Full stage-level decomposition}

\begin{table}[htbp]
\centering
\caption{Full operational cost decomposition. The non-evaluation residual is observed wall time
minus logged evaluation time; it bundles model update, setup, and checkpointing and is not a
training-time measurement.}
\label{tab:cost-full}
\small
\begin{tabularx}{\textwidth}{@{}L L c c@{}}
\toprule
\textbf{Component} & \textbf{Measured time / scale} & \textbf{Ext.\ calls} & \textbf{Per req.?} \\
\midrule
Fact extraction & 4{,}005 QA $\rightarrow$ 11{,}786 triples (runtime not instrumented) & $\approx$4{,}005 nominal & No \\
Global graph construction & 4{,}005 nodes; 45{,}683 edges (runtime not instrumented) & 0 & No \\
Optional GradAlign preprocessing & 62.99\,s / 1{,}900 samples ($\approx$30.2/s) & 0 & No \\
Request-conditioned graph targeting & 11.4--33.4\,s (cache-hit) & 0 & \textbf{Yes} \\
Observed non-evaluation residual & $\approx$5.7--6.9\,min & 0 & Yes \\
Lightweight checkpoint evaluation & 5.1--6.6\,min & 0 & Dev-time \\
Full adversarial route audit & 63.0--83.1\,min; 4{,}464--5{,}376 local gen. & 0 & No \\
\bottomrule
\end{tabularx}
\end{table}

With cached artefacts, request-conditioned targeting required 11.4\,s (partial deletion), 33.0\,s
(entity and instance), and 33.4\,s (complete), averaging 25.9\,s. A matched Seed-Only runtime log was
not available, so Seed-Only is omitted from the operational comparison. For completeness---these are
full end-to-end workflow times under differing audit schedules, not a controlled speed comparison---raw
observed wall times were 5.85, 7.63, and 7.70\,h for \method{} and 5.49, 6.90, and 7.03\,h for DPO, on
complete, entity, and partial deletion respectively.

\subsection{Graph scale and sparsification}

\begin{table}[htbp]
\centering
\caption{Original graph versus the final sparse (mutual-kNN) graph with partial GradAlign
augmentation, on the 4{,}005-node TOFU corpus.}
\label{tab:scale}
\small
\begin{tabular}{@{}p{4.6cm}ccc@{}}
\toprule
\textbf{Metric} & \textbf{Original} & \textbf{Final} & \textbf{Change} \\
\midrule
Nodes & 4{,}005 & 4{,}005 & 0 \\
Undirected edges & 52{,}816 & 45{,}683 & $-13.51\%$ \\
Average degree & 26.38 & 22.81 & $-13.51\%$ \\
95th-percentile degree & 42 & 30 & $-28.57\%$ \\
Maximum degree & 112 & 30 & $-73.21\%$ \\
Density & 0.659\% & 0.570\% & lower \\
Connected components & 1 & 1 & 0 \\
Isolated nodes & 0 & 0 & 0 \\
\bottomrule
\end{tabular}
\end{table}

The extracted facts (11{,}786 triples; 1{,}805 unique heads, 1{,}189 relations, 5{,}756 tails) and
the final graph are persisted and loaded at request time rather than reconstructed, amortising
construction cost across requests. The edge file and a representative GradAlign cache occupy
approximately 7.81\,MB; extracted facts and other metadata are persisted separately. These results
are structural scalability indicators at one corpus size and do not constitute a multi-corpus-size
scaling benchmark.

\textbf{Maintainability (cache validity).} As a deployment requirement, cached facts, embeddings,
graph edges, and GradAlign signatures should be versioned against the corpus snapshot, extraction
model, embedding model, and graph configuration; a corpus or model update requires rebuilding the
affected artefacts before subsequent deletion requests.

\subsection{GradAlign characterisation and provenance}
\label{sec:grad}

GradAlign is a \emph{representation-gradient alignment proxy}: it computes the gradient of the
answer-token cross-entropy with respect to the final-layer hidden representation, L2-normalises it
per sample, and scores edges by clipped cosine similarity. It is not full parameter-gradient
similarity. GradAlign is an \emph{optional} component and is not claimed as an independent empirical
contribution.

\begin{table}[htp]
\centering
\caption{GradAlign cache and edge statistics for the representative artefact (GPT-2-medium,
1{,}024-dimensional representations).}
\label{tab:gradalign}
\small
\begin{tabular}{@{}p{7.1cm}c@{}}
\toprule
\textbf{Metric} & \textbf{Value} \\
\midrule
Cached signatures (1{,}024-dim float16; 0 unusable) & 1{,}991 \\
Cache size & 4.07\,MB \\
Edges with both endpoint signatures & 17{,}108 (37.45\%) \\
Edges with non-zero GradAlign & 16{,}102 (35.25\%) \\
Mean / median GradAlign (affected edges) & 0.301 / 0.264 \\
90th / 95th percentile (affected edges) & 0.596 / 0.702 \\
Mean GradAlign share of combined weight (affected edges) & 21.12\% \\
\bottomrule
\end{tabular}
\end{table}

On the edges where it is defined, GradAlign contributes approximately one-fifth of the combined edge
weight on average (its contribution depends on the fixed coefficient $\lambda=0.7$). The
representative cache was constructed around the \emph{complete}-deletion seed neighbourhood
(1{,}991 signatures), giving full coverage for complete deletion (100\%) and partial coverage for the
partial (45.2\%) and entity/instance (83.5\%) settings; edges outside the cached subset receive a
GradAlign score of zero. GradAlign is an optional component, and we report these statistics only to
characterise the signal: we \textbf{make no cross-task GradAlign effectiveness claim}, which would
require uniform per-task caches.

% \subsection{Reliability controls}

% \begin{itemize}
% \item \textbf{Frozen evaluation manifests}: fixed sample and route sets, recorded for all three tasks.
% \item \textbf{Deterministic environment}: seed 42 and hardware metadata recorded; local-files-only model loading prevents version drift.
% \item \textbf{Bounded support expansion}: mutual-kNN ($K_{\mathrm{edge}}=30$), 1-/2-hop closure, top-$k$ caps, personalised PageRank with bounded top-60/min-15 support, and a fixed 64-item retain frontier; selected support sets contained 46--145 neighbours.
% \item \textbf{Staged graph activation}: a seed-only warm-up precedes graph-enabled steps (see the core implementation settings, Table~\ref{tab:settings}). A measured benefit is not claimed; an ablation is needed.
% \item \textbf{Actionability and retain-safety gates}: ambiguous neighbours are excluded rather than auto-forgotten or auto-retained.
% \item \textbf{Automated edge-integrity audit}: 0 self-loops, 0 duplicate edges, 0 non-finite values, 0 out-of-range components, 0 weight-formula mismatches.
% \item \textbf{Rule-based adversarial route prompts}: direct, paraphrase, indirect, cloze, related-fact, list-summary, relation-inversion, and entity-alias routes generated offline, incurring no external-LLM cost.
% \end{itemize}

\subsection{Evaluation-cost optimization}

In the recorded RTX 3090 runs, logged evaluation accounted for 98.0--98.8\% of observed wall time,
confirming that evaluation cadence---not support selection---dominates \method{}'s runtime. A hybrid
schedule (frequent lightweight evaluation; full route audit at selected milestones) used 26{,}880
adversarial generations and 7.70\,h on partial deletion, versus 79{,}200 generations and 16.73\,h
under a full-audit schedule---66.1\% fewer generations and 54.0\% lower wall time. Because the two
runs were not otherwise identical, this is evidence that \emph{audit cadence is a major operational
cost lever}, not a controlled algorithmic speedup.

\subsection{Measurement scope}

\begin{itemize}
\item The model-update figure is an observed non-evaluation residual (wall time minus logged evaluation), not a pure training-time measurement.
\item GradAlign is optional and its representative cache covers the complete-deletion neighbourhood (\S\ref{sec:grad}); we therefore make no cross-task GradAlign effectiveness claim.
\item Per-generation audit cost is observed throughput, not normalised for generated length or batching.
\item The reliability evidence concerns reproducibility, artefact integrity, bounded execution, and evaluation consistency; it does not constitute a statistical variance analysis across random seeds (all results use a single seed).
\end{itemize}


==> implementation_details.tex <==
In our experiments, we
set $\rho=0.15$ and iterate until the $L_1$ change is below $10^{-8}$,
with a maximum of 200 iterations. 
